Humanizing the Machine: Proxy Attacks to Mislead LLM Detectors

The advent of large language models (LLMs) has revolutionized the field of text generation, producing outputs that closely mimic human-like writing. Although academic and industrial institutions have developed detectors to prevent the malicious usage of LLM-generated texts, other research has doubt about the robustness of these systems. To stress test these detectors, we introduce a proxy-attack strategy that effortlessly compromises LLMs, causing them to produce outputs that align with human-written text and mislead detection systems. Our method attacks the source model by leveraging a reinforcement learning (RL) fine-tuned humanized small language model (SLM) in the decoding phase. Through an in-depth analysis, we demonstrate that our attack strategy is capable of generating responses that are indistinguishable to detectors, preventing them from differentiating between machine-generated and human-written text. We conduct systematic evaluations on extensive datasets using proxy-attacked open-source models, including Llama2-13B, Llama3-70B, and Mixtral-8*7B in both white- and black-box settings. Our findings show that the proxy-attack strategy effectively deceives the leading detectors, resulting in an average AUROC drop of 70.4% across multiple datasets, with a maximum drop of 90.3% on a single dataset. Furthermore, in cross-discipline scenarios, our strategy also bypasses these detectors, leading to a significant relative decrease of up to 90.9%, while in cross-language scenario, the drop reaches 91.3%. Despite our proxy-attack strategy successfully bypassing the detectors with such significant relative drops, we find that the generation quality of the attacked models remains preserved, even within a modest utility budget, when compared to the text produced by the original, unattacked source model.

==> secs/limitation.tex <==
\section{Limitation and Discussion}
\label{sec:limit}


==> tables/cross_discipline_auc.tex <==
\begin{table}[t]
  \small
  \caption{AUROCs of detectors in on the texts generated by different models on the cross-discipline dataset. CS$\rightarrow$PHX, PHX$\rightarrow$HSS. }
\label{tab:cross_discipline_auroc}
  \begin{center}
  
  \centerline{
  \setlength\tabcolsep{0.5pt}
  \begin{tabular}{c|c|cc|cc|cc}
    \toprule
    \multirow{2}{*}{Dataset}& \multirow{2}{*}{Models$\rightarrow $} &\multirow{2}{*}{Llama2-13B} & 
    \modelname
    & \multirow{2}{*}{Llama3-70B} & \modelname

    & \multirow{2}{*}{Mixtral-8x7B}
 & \modelname \\

 & & & 
    (Llama2-7B)
    &  & (Llama3-8B)

    & 
 & (Mistral-7B) \\
 \hline
 \multirow{23}{*}{CS$\rightarrow$PHX} 
&\multicolumn{7}{>{\columncolor{gray!20}}c}{The Generation Utility}\\
 &$S_{\text{Bert}}$ &0.8351 &0.8308  & 0.8118 & 0.8034 &0.8057  & 0.7888\\
 &ROUGE-1 &0.2972&0.2965& 0.2992&0.2712  &0.2330  & 0.2045\\
 &ROUGE-2 &0.0831 & 0.0783 &0.0782&0.0770  &0.0641  & 0.0505\\
 &ROUGE-L &0.1700 &0.1620 &0.1602&0.1543  & 0.1369 & 0.1204\\
   &\multicolumn{7}{>{\columncolor{gray!20}}c}{The White-box Setting}\\
     &Likelihood & 0.9999& 0.8376 & 0.9974& 0.6348&0.6630 & 0.2604\\
    %\hline
    &LogRank &0.9982 & 0.7999 &0.9932 & 0.5553&0.6533 &0.2354
\\
    &LRR &0.4277 &0.3563  &0.2588 & 0.1800&0.5065 &0.1505
\\
    &NPR &0.9781 & 0.8403 &0.9859 &0.7343 &0.7955 &0.5706
\\
    &DNA-GPT & 0.9884& 0.6653 &0.9943 &0.4812 & 0.6001&0.1513
    \\
    &DetectGPT &0.5784 & 0.5996 &0.4987 &0.4131&0.2568 &0.1778
    \\
    &Fast-DetectGPT &0.9978 &0.9881  & 0.9999&0.9799 &0.8390 &0.1319
    \\ 
&\multicolumn{7}{>{\columncolor{gray!20}}c}{The Black-box Setting}\\
&Roberta-base & 0.8718& 0.7801 &0.7535 &0.4775 &0.7379 &0.6387
\\
 &Roberta-large &0.8132 &0.7183  & 0.6495&0.4435 & 0.7339&0.6343
\\
    &Likelihood(Neo-2.7) & 0.8185& 0.5475 & 0.9351&0.3526 &0.3199 &0.0928
\\
    %\hline
    &LogRank(Neo-2.7) &0.8226 & 0.5458 &0.9309 & 0.3078&0.2848 &0.0691 \\
    &LRR(Neo-2.7) &0.7536 & 0.5125 &0.8463 &0.1807 & 0.2328&0.0369
\\
    &NPR(Neo-2.7) &0.5517 &0.4396  &0.6458 & 0.4298& 0.5210 & 0.3357
\\
    &DNA-GPT(Neo-2.7) & 0.8078& 0.3820 &0.9004 &0.2909 &0.4249 &0.1130
    \\
    &DetectGPT(T5-3B/Neo-2.7) & 0.1697 & 0.1877 &0.2994 &0.2673 & 0.2516& 0.1958
    \\
    &Fast-DetectGPT(GPT-J/Neo-2.7) & 0.9673&  0.6714& 0.9759& 0.3919& 0.4697&0.0427
\\
\hline\hline
 \multirow{24}{*}{PHX$\rightarrow$HSS}
 &\multicolumn{7}{>{\columncolor{gray!20}}c}{The Generation Utility}\\
 &$S_{\text{Bert}}$ &0.8291 & 0.8201 &0.8007  & 0.7976 & 0.8105 &0.7997 \\
 &ROUGE-1 &0.2632 & 0.2385 & 0.2506 & 0.2277 & 0.2381 &0.2104\\
 &ROUGE-2 &0.0535 &0.0459  & 0.0513 & 0.0448 & 0.0447 &0.0364\\
 &ROUGE-L & 0.1470& 0.1315 & 0.1383 & 0.1299 &0.1334  &0.1178\\
    %\cline{2-8}
    &\multicolumn{7}{>{\columncolor{gray!20}}c}{The White-box Setting}\\
    &Likelihood & 1.0000& 0.8706 &0.9999 & 0.8317& 0.8145&0.4925
 \\
    %\hline
    &LogRank & 0.9997& 0.8575 &0.9976 & 0.7842& 0.8244&0.4670
 \\
    &LRR & 0.8096& 0.6536 &0.4530 &\best{0.3323} &0.7862 &0.3387
\\
    &NPR &0.9993 & \worst{0.9414} &0.9954 &\worst{0.9327} &0.9226
 &0.8313
 \\
    &DNA-GPT &0.9622 & \best{0.7278} &0.9985 &0.7534 &0.6946
 &\best{0.2822}
    \\
    &DetectGPT & 0.9338&  0.8306& 0.9170&0.8081 & 0.5982&\worst{0.5796}
    \\
    &Fast-DetectGPT &0.9965 & 0.9365 & 0.9961& 0.9739&0.9700 &0.5333
    \\ 
&\multicolumn{7}{>{\columncolor{gray!20}}c}{The Black-box Setting}\\
&Roberta-base & 0.8550&  \worst{0.7608}&0.7399 &0.6119 &0.6895 &0.5583
\\
 &Roberta-large & 0.8304& 0.7291 &0.7298 & 0.5819& 0.6733&\worst{0.5934}
\\
    &Likelihood(Neo-2.7) &0.9590 & 0.7121 &0.9403 & 0.5987&0.6679 &0.3149
 \\
    %\hline
    &LogRank(Neo-2.7) &0.9617 & 0.7057 &0.9343 & 0.5553& 0.6587&0.2879
 \\
    &LRR(Neo-2.7) & 0.9384& 0.6624 &0.8717 &\best{0.3780} &0.5816 &0.2153
 \\
    &NPR(Neo-2.7) &0.9422 & 0.7511 &0.9226 &0.7528 &0.8010 &0.6218
 \\
    &DNA-GPT(Neo-2.7) & 0.9113&  \best{0.5827}& 0.9672& 0.5760& 0.6320&
   \best{0.2082} \\
    &DetectGPT(T5-3B/Neo-2.7) & 0.8160 & 0.6510 & 0.8026&\worst{0.6788} & 0.6993&0.5371\\
    &Fast-DetectGPT(GPT-J/Neo-2.7) &0.9891 & 0.7488 &0.9839 & 0.6296& 0.7827&0.5333
    \bottomrule
  \end{tabular}
  }
  \end{center}
  \vskip -10pt
\end{table}
